Multi-objective Explanations of GNN Predictions

Graph Neural Network (GNN) has achieved state-of-the-art performance in various high-stake prediction tasks, but multiple layers of aggregations on graphs with irregular structures make GNN a less interpretable model. Prior methods use simpler subgraphs to simulate the full model, or counterfactuals to identify the causes of a prediction. The two families of approaches aim at two distinct objectives, "simulatability" and "counterfactual relevance", but it is not clear how the objectives can jointly influence the human understanding of an explanation. We design a user study to investigate such joint effects and use the findings to design a multi-objective optimization (MOO) algorithm to find Pareto optimal explanations that are well-balanced in simulatability and counterfactual. Since the target model can be of any GNN variants and may not be accessible due to privacy concerns, we design a search algorithm using zeroth-order information without accessing the architecture and parameters of the target model. Quantitative experiments on nine graphs from four applications demonstrate that the Pareto efficient explanations dominate single-objective baselines that use first-order continuous optimization or discrete combinatorial search. The explanations are further evaluated in robustness and sensitivity to show their capability of revealing convincing causes while being cautious about the possible confounders. The diverse dominating counterfactuals can certify the feasibility of algorithmic recourse, that can potentially promote algorithmic fairness where humans are participating in the decision-making using GNN.

==> confounder.tex <==
\subsection{Proof of confounders}
% Given a GNN model with $L$ layers,
% we have an explanation subgraph $G_i$ to explain $v_i$.
% The perturbation, $\tilde{G}_i$, is obtained by removing $\Delta(G_i, \tilde{G}_i)$ from $G_i$,
% and prediction of $v_i$ in $G_i$ (and $\tilde{G}_i$) is $\mathbf{y}_i^\prime$ (and $\tilde{\mathbf{y}}_i^\prime$).
% Mathematically, 
% confounders are defined by $\{c| c \in \cap_{u\in \{ v_i, \Delta(G_i, \tilde{G}_i) \} } \cup_{l=1}^L\mathcal{N}_l{(u)}  \}$.

% Based on Eq.(\ref{eq:message},\ref{eq:aggregate},\ref{eq:hidden}),
% the representation of node $v_i$ at the $l$-th layer, $h_i^{(l)}$, can be formulated as:
% \begin{equation}
% \begin{aligned}
%     h_i^{(l)} 
%     & = \textnormal{UPDATE}(\textnormal{AGG}(\textnormal{MSG}(h_j^{(l-1)},h_i^{(l-1)})|v_j\in\mathcal{N}(v_i)),\theta^{(l)}) \\
%     & \triangleq f^{(l)}(h_j^{(l-1)},h_i^{(l-1)}, \theta^{(l)} |v_j\in\mathcal{N}(v_i)) \\
%     & = f^{(l-m+1)}(h_j^{(l-m)}, \theta^{(l-m+1)} |v_j\in\mathcal{N}_{\leq m}(v_i)), 1\leq m\leq l,
% \end{aligned}
% \end{equation}
% where $\mathcal{N}_{\leq m}(v_i)$ is the entire $m$-hop neighborhoods of $v_i$, e.g., including $v_i$ and any other nodes within $m$-hop away from $v_i$.
% Clearly, $h_i^{(l)}$ is defined by its $m$-hop neighbors' representation at the $(l-m+1)$-th layer.
% Specifically, when taking $m=l$, we have
% $h_i^{(l)}=f^{(1)}(h_i^{(0)},\theta^{(1)}|v_j\in\mathcal{N}_{\leq l}(v_i))$.

We prove the existence of confounder in the explanations generated by the proposed algorithm on GNN.

\begin{thm}

Consider an $L$-layer GNN, and each layer takes
\begin{eqnarray}
\mathbf{m}_{ji}^{(l)}&=&\mathbf{h}_{j}^{(l-1)},\label{eq:sem1}\\
\mathbf{a}_i^{(l)}&=&\sum_{v_i \cup \mathcal{N}(v_i)} \mathbf{m}_{ji}^{(l)},\label{eq:sem2}\\
\mathbf{h}_i^{(l)} &=&\sigma((\boldsymbol{\theta}^{(l)})^{\top} \mathbf{a}^{(l)}_i)\label{eq:sem3},
\end{eqnarray}
for $l=1,\dots, L$.
Confounders in the explanation $G_i$ of the node $v_i$ are the nodes that are within $L$-hops away from $v_i$ and that remain in the counterfactual $\tilde{G}_i$:
\begin{equation}
\{c| c \in \cup_{l=1}^L\mathcal{N}_l{(v_i)}, c\notin \Delta(G_i, \tilde{G}_i)  \},
\end{equation}
where $\mathcal{N}_l(v_i)$ contains all nodes $l$-hop away from $v_i$.
\end{thm}

\begin{proof}
Let the ``fact'' $G_i$ be the subgraph explanation and the ``counterfactual'' $\tilde{G}_i$ be $G_i\setminus \Delta$, where $\Delta$ is a portion removed from $G_i$.
Unless $\Delta$ is $G_i\setminus \{v_i\}$ (that is, $\tilde{G}_i$ contains $v_i$ only),
there will be more than one messages getting into $a_i^{(l)}$ for all layer $l$ ($h_{i}^{(l-1)}$ always participates in the computation of $h_i^{(l)}$).
Since we constrain the explanations $G_i$ to be an acyclic graph (tree),
the messages emitting from any node from $\Delta$ will be removed from the right hand side of the SEM Eq. (\ref{eq:sem2}).
% Since there is no other path that the removed nodes can pass messages to $\mathbf{h}_i^{l}$ on any level $l$,
But if we assume that there are more than one messages that appear in Eq. (\ref{eq:sem2}),
the remaining messages after removing $\Delta$ will still participate in the computation of $\mathbf{h}_i^{(L)}$, whose value will be conditioned on these remaining messages.

Therefore, the effect of removing $\Delta$ on $\mathbf{h}_i^{(L)}$ is confounded by other inputs that are within $L$-hops from $v_i$ and are not in $\Delta$.
Any other nodes that are either more than $L$-hops away from $v_i$ or within $\Delta$ will participate in the computation $\mathbf{h}_i^{L}$ after $\Delta$ is removed.
\end{proof}

We have the following example to demonstrate the theorem.
Figure \ref{fig:gi_example} shows a chain $G_i$ containing $(2-1-i-3)$ extracted to explain the target node $i$, and $\Delta=\{2\}$ will be removed to construct a counterfactual $G_i\setminus \{2\}$.
We show the computation graph that executes the computation of the SEM.
Each node represents $h^{(l)}_i$ in the $l$-th GNN layer, and edge indicates the dependencies of the node on other nodes.
Let $L=2$.
Expanding the output on node $i$ on the last layer of GNN:
\begin{equation}
\begin{aligned}
\label{eq:sem}
    \textbf{h}_i^{(2)} 
    &= 
    \sigma((\boldsymbol{\theta}^{(2)})^\top \textbf{a}_i^{(2)}) \\
    &= 
    \sigma((\boldsymbol{\theta}^{(2)})^\top \sum_{v_j \in \{v_i \cup \mathcal{N}(v_i) \} } \mathbf{m}_{ji}^{(2)} ) \\
    &= 
    \sigma((\boldsymbol{\theta}^{(2)})^\top \sum_{v_j \in \{v_i \cup \mathcal{N}(v_i) \}} \mathbf{h}_{j}^{(1)} ) \\
    &= 
    \sigma((\boldsymbol{\theta}^{(2)})^\top \sum_{v_j \in \{v_i \cup \mathcal{N}(v_i) \}} \sigma((\boldsymbol{\theta}^{(1)})^\top \textbf{a}_j^{(1)})) \\
    &= 
    \sigma((\boldsymbol{\theta}^{(2)})^\top \sum_{v_j \in \{v_i \cup \mathcal{N}(v_i) \}}
    \sigma((\boldsymbol{\theta}^{(1)})^\top \sum_{v_k \in \{v_j \cup \mathcal{N}(v_j) \}} \mathbf{m}_{kj}^{(1)} )) \\
    &= 
    \sigma((\boldsymbol{\theta}^{(2)})^\top \sum_{v_j \in \{v_i \cup \mathcal{N}(v_i) \}}
    \sigma((\boldsymbol{\theta}^{(1)})^\top \sum_{v_k \in \{v_j \cup \mathcal{N}(v_j) \}} \textbf{h}_k^{(0)} )) \\
\end{aligned}
\end{equation}

Based on Eq. (\ref{eq:sem}), 
we explicitly show the SEM based on the structure of $G_i$ and GNN model. 
Obviously, when $\Delta$ is retained in $G_i$ ($do(\cup \Delta)$), target node $i$'s representation is defined by its 2-hop neighborhoods as:
\begin{equation}
\begin{aligned}
\textbf{h}_{i|do(\cup\Delta)}^{(2)} = 
\sigma[ (\boldsymbol{\theta}^{(2)})^\top 
 (& \sigma((\boldsymbol{\theta}^{(1)})^\top (\textbf{h}^{(0)}_i + \textbf{h}^{(0)}_1 + \textbf{h}^{(0)}_3 ) ) \\
 +& \sigma((\boldsymbol{\theta}^{(1)})^\top (\textbf{h}^{(0)}_i + \textbf{h}^{(0)}_1 + \textbf{h}^{(0)}_2 ) ) \\
 +& \sigma((\boldsymbol{\theta}^{(1)})^\top (\textbf{h}^{(0)}_i +\textbf{h}^{(0)}_3)))
 ].
\end{aligned}
\end{equation}
When $\Delta$ is removed from $G_i$ ($do(\setminus\Delta)$,
we have $\tilde{G}_i$ and the corresponding new representation of $\mathbf{h}_i^{(2)}$:
\begin{equation}
\begin{aligned}
\textbf{h}_{i|do(\setminus\Delta)}^{(2)} = 
\sigma[ (\boldsymbol{\theta}^{(2)})^\top 
 (& \sigma((\boldsymbol{\theta}^{(1)})^\top (\textbf{h}^{(0)}_i + \textbf{h}^{(0)}_1 + \textbf{h}^{(0)}_3 ) )\\
 +& \sigma((\boldsymbol{\theta}^{(1)})^\top (\textbf{h}^{(0)}_i + \textbf{h}^{(0)}_1 ))\\
 +& \sigma((\boldsymbol{\theta}^{(1)})^\top (\textbf{h}^{(0)}_i + \textbf{h}^{(0)}_3))
 ],
\end{aligned}
\end{equation}

The impact of removing $\Delta$ is then $\Delta \textbf{h}_i^{(2)}=\textbf{h}_{i|do(\cup\Delta)}^{(2)}-\textbf{h}_{i|do(\setminus\Delta)}^{(2)}$.

Assume that all $\mathbf{h}$'s and $\boldsymbol{\theta}$'s are scalars (denoted by $h$ and $\theta$).
Setting $\theta^{(1)}=\theta^{(2)}=1$, 
$h_i^{(0)}=0, h_1^{(0)}=0$ and $h_2^{(0)}=1$,
the impact of $h^{(0)}_3$ to $\Delta h_i^{(2)}$ is
\begin{equation}
\begin{aligned}
    \Delta h_i^{(2)} =& \sigma (\sigma(h^{(0)}_3) +\sigma(1) + \sigma(h_3^{(0)})) \\
    &- \sigma(\sigma(h^{(0)}_3) + \sigma(0) + \sigma(h^{(0)}_3) ).
\end{aligned}
\end{equation}
% Similarly, when setting $h_A^{(0)}=0$, the impact of $h^{(0)}_C$ to $\Delta h_X^{(2)}$ is
% \begin{equation}
% \begin{aligned}
%     \Delta h_X^{(2)}=&
%     \sigma(\sigma(h^{(0)}_C)+\sigma(1) + \sigma(h^{(0)}_C)) \\
%     &- \sigma(\sigma(h^{(0)}_C)+\sigma(0)+\sigma(h^{(0)}_C)).
% \end{aligned}
% \end{equation}
$\Delta h^{(2)}_i$ is then affected by input from node $1$, which indicates node $3$ confounds with the effect of removing $\Delta=\{2\}$. 
% In Figure
% Therefore, we can generate a Structural Equation Model (SEM) to explicitly describe the relations between variables, , as shown in Figure \ref{fig:gi_sample}.
% Nodes in SEM represent either latent variables or measured variables, 
% and edges with weights indicate the potential causal dependencies between variables.
% The weights vary when using different AGG functions, 
% for example, 
% ``element-wise sum (or average)" assigns 1 (or $\frac{1}{|\mathcal{N}|}$) to all edges, 
% while it assigns weights according to the attention mechanism in GAT \cite{velivckovic2018gat}.
% \begin{figure}[h]
% \label{}
% \centering
%     \includegraphics[width=0.45\textwidth]{pic/gi_example.pdf}%
%     \caption{\small
%     \textit{Left}: A sample of $G_i$ explaining $X$ and the structural equations to compute $h_i^{(l)}$ for each layer $l$, with summation as the message aggregation.
%     $B$ is the node to be removed from $G_i$ to obtain the counterfactual $G_i^\prime$.
%     \textit{Right}: rolling out the structural equation in a computation graph.
%     Arrows are information flow
%     and the darker ones highlight the messages flowing into $h^{(2)}_X$.
%     The treatment $do(\setminus B)$ causes $m_{BA}^{(l)}=0$ for $l=1,2$.
%     The numbers alongside the computation nodes show that different values of $C$ ($0$ and $1$) 
%     influence how the treatment change the outcome ($h^{(l)}_{X|do(\cup B)}-h^{(l)}_{X|do(\setminus B)}$).
%     % e.g., 
%     % when $C$ takes value 0 (or 1), what is the corresponding $\Delta h^{(l)}_X$.
%     }
%     % and the removal of node $B$ constructs the counterfactual $\tilde{G}_i$.}
%     \label{fig:gi_sample}
% \end{figure}


==> prior_works.tex <==
19ICML WORKSHOP 
Explainability Techniques for Graph Convolutional Networks
adopts three techniques to explain the predictions made by GNN:
(1)Sensitivity Analysis (SA)
produces a saliency map using gradients.
(2)Guided Backpropagation (GBP)
also constructs a saliency map using gradients while negative gradients are clipped during backpropagation.
(3)Layer-wise Relevance Propagation (LRP)
produces relevance maps by decomposing the output signal of every transformation into a combination of its inputs.
In general, these methods are based on gradients and
they are all existing methods which are first applied to GNN explanations.
They can be applied to both node classification and graph classification.

19CVPR
Explainability Methods for Graph Convolutional Neural Networks
adopts two techniques to explain the predictions made by GNN:
(1)Class Activation Mapping (CAM) and gradient-weighted CAM (Grad-CAM)
identify important, class-specific features at the last convolutional layer as opposed to the input space.
(2)Excitation Backpropagation (EB) and contrastive EB
ignore non-linearities in the backward-pass through the network, 
and are able to generate heat-maps that “conserve” evidence for or against a network predicting any particular class
In general, these methods are based on gradients and
they are all existing methods which are first applied to GNN explanations.
They can be applied to both only graph classification.

19NIPS
GNNExplainer: Generating Explanations for Graph Neural Networks
identifies a compact subgraph structure and a small subset of node features that have a crucial role in GNN’s prediction.
GnnExplainer is formalized as an optimization task that maximizes the mutual information between the prediction of the full model and the prediction of simplified explainer model.
The parameters of the explainer model include 
the feature mask parameters and the adjacency matrix mask parameters.
If it is a node classification task,
it extracts n-hop neighbors of the target node to be explained,
while the whole graph is used for graph classification task.
In general, 
the explainer model is trained to approximate the output of the full model, and finally the weights of the explainer model are extracted for explanations.


20
GraphLIME: Local Interpretable Model Explanations for Graph Neural Networks
identifies K most representative features as the explanations for node classification task.
A nonlinear interpretable model is trained from n-hop neighbors of the target node to be explained.
The Hilbert-Schmidt Independence Criterion (HSIC) Lasso is used to  compute the K most representative features,
which is a nonlinear feature selection method.
In general, 
the local non-linear interpretable model is trained for feature selection,
and top K important features are selected for explanations.


20KDD
XGNN: Towards Model-Level Explanations of Graph Neural Networks
identifies a salient subgraph structure as the explanations for graph classification task.
A graph generator is trained by policy gradient method based on reinforcement learning,
which generate subgraphs that approximate the predictions of the full model.
In general, 
the graph generator is trained using reinforcement learning,
and salient subgraphs are generated for explanations.

NIPS 2015
Convolutional networks on graphs for learning molecular fingerprints
Section 4.1 produces interpretation of the GCN for molecule classification.

In conclusion,
existing methods are divided in two types.
One is based on gradients,
where the gradient is used to find out the most important factors affecting the predictions.
The other is based on explainer models,
where an explainer model is trained to help find the most important factors.
Our approach is search-based, 
different from both of them, 
and is thought to be more human-friendly.


==> survey_question/case11-12.tex <==



==> survey_question/case3-4.tex <==
\begin{questionblock}
\vspace*{-110pt}
\begin{figure}[H]
\centering
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case3_1.pdf}%
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case3_5.pdf}\\
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case3_2.pdf}%
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case3_6.pdf}\\
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case3_3.pdf}%
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case3_7.pdf}\\
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case3_4.pdf}%
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case3_8.pdf}\\
    % \caption{\small Explanations with different simulatability and counterfactual relevance of GNN predictions.}
% \hspace{50pt}
\end{figure}

% \small Answer the following three questions:
\begin{itemize}
    \scriptsize
    \item (\textit{\textcolor{red}{Simulatability}}) How well do you think the second subgraph $G$2 is reproducing the prediction computed in the first graph $G$1. \textcolor{blue}{(1-very little,2-little,3-not sure,4-a little, 5-very well)}.
    \item (\textit{\textcolor{red}{Counterfactual}}) How much do you think the removed component in the third subgraph $G$3 causes the search engine to predict the class distribution in the second subgraph $G$2, had it not been removed? \textcolor{blue}{(1-very little,2-little,3-not sure,4-a little, 5-very much)}.
    \item (\textit{\textcolor{red}{Counterfactual}}) How much do you think the removed component in the forth subgraph $G$4 causes the search engine to predict the class distribution in the second subgraph $G$2, had it not been removed? \textcolor{blue}{(1-very little,2-little,3-not sure,4-a little, 5-very much)}.
    \item (\textit{\textcolor{red}{Adoption of the explanation}}) How much will you accept the search engine's computation of the probabilities, if they were computed on the second smaller subgraph $G$2 rather than the first larger subgraph $G$1? \textcolor{blue}{(1-very little, 2-little,3-not sure,4-a little, 5-very much)}.
\end{itemize}
\end{questionblock}

\begin{questionblock}
\vspace*{-110pt}
\begin{figure}[H]
\centering
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case4_1.pdf}%
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case4_5.pdf}\\
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case4_2.pdf}%
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case4_6.pdf}\\
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case4_3.pdf}%
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case4_7.pdf}\\
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case4_4.pdf}%
    \includegraphics[width=0.5\textwidth]{pic/survey_fig/case4_8.pdf}\\
    % \caption{\small Explanations with different simulatability and counterfactual relevance of GNN predictions.}
% \hspace{50pt}
\end{figure}

% \small Answer the following three questions:
\begin{itemize}
    \scriptsize
    \item (\textit{\textcolor{red}{Simulatability}}) How well do you think the second subgraph $G$2 is reproducing the prediction computed in the first graph $G$1. \textcolor{blue}{(1-very little,2-little,3-not sure,4-a little, 5-very well)}.
    \item (\textit{\textcolor{red}{Counterfactual}}) How much do you think the removed component in the third subgraph $G$3 causes the search engine to predict the class distribution in the second subgraph $G$2, had it not been removed? \textcolor{blue}{(1-very little,2-little,3-not sure,4-a little, 5-very much)}.
    \item (\textit{\textcolor{red}{Counterfactual}}) How much do you think the removed component in the forth subgraph $G$4 causes the search engine to predict the class distribution in the second subgraph $G$2, had it not been removed? \textcolor{blue}{(1-very little,2-little,3-not sure,4-a little, 5-very much)}.
    \item (\textit{\textcolor{red}{Adoption of the explanation}}) How much will you accept the search engine's computation of the probabilities, if they were computed on the second smaller subgraph $G$2 rather than the first larger subgraph $G$1? \textcolor{blue}{(1-very little, 2-little,3-not sure,4-a little, 5-very much)}.
\end{itemize}

\end{questionblock}


==> survey_question/case5-6.tex <==



==> survey_question/case7-8.tex <==



==> survey_question/case9-10.tex <==


